The three-dimensional structure of the Eta Carinae Homunculus

We investigate, using the modeling code SHAPE, the three-dimensional structure of the bipolar Homunculus nebula surrounding Eta Carinae, as mapped by new ESO VLT/X-Shooter observations of the H2 $\lambda=2.12125$ micron emission line. Our results reveal for the first time important deviations from the axisymmetric bipolar morphology: 1) circumpolar trenches in each lobe positioned point-symmetrically from the center and 2) off-planar protrusions in the equatorial region from each lobe at longitudinal (~55 degrees) and latitudinal (10-20 degrees) distances from the projected apastron direction of the binary orbit. The angular distance between the protrusions (~110 degrees) is similar to the angular extent of each polar trench (~130 degrees) and nearly equal to the opening angle of the wind-wind collision cavity (~110 degrees). As in previous studies, we confirm a hole near the centre of each polar lobe and no detectable near-IR H2 emission from the thin optical skirt seen prominently in visible imagery. We conclude that the interaction between the outflows and/or radiation from the central binary stars and their orientation in space has had, and possibly still has, a strong influence on the Homunculus. This implies that prevailing theoretical models of the Homunculus are incomplete as most assume a single star origin that produces an axisymmetric nebula. We discuss how the newly found features might be related to the Homunculus ejection, the central binary and the interacting stellar winds. We also include a 3D printable version of our Homunculus model.

==> views.tex <==
VIEW={Initial}
  COO=-0.06521779298782349 0.39206594228744507 -0.12889957427978516
  C2C=-0.06051350384950638 0.6740224957466125 0.7362279891967773
  ROO=9.31
  ROLL=127.43660402458738
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END
VIEW={Wireframe}
   COO=-0.06521779298782349 0.39206594228744507 -0.12889957427978516
  C2C=-0.06051350384950638 0.6740224957466125 0.7362279891967773
  ROO=9.31
  ROLL=127.43660402458738
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=HiddenWireframe
END
VIEW={Flipped}
  COO=-0.06521892547607422 0.39206287264823914 -0.12890379130840302
  C2C=-0.031322404742240906 -0.6797863841056824 -0.7327410578727722
  ROO=9.31
  ROLL=-54.666115701492394
  AAC=60.000001669652114
  BGCOLOR=1.000000 1.000000 1.000000
  LIGHTS=CAD
  RENDERMODE=Solid
END

